Learning Hierarchically Structured Concepts

We study the question of how concepts that have structure get represented in the brain. Specifically, we introduce a model for hierarchically structured concepts and we show how a biologically plausible neural network can recognize these concepts, and how it can learn them in the first place. Our main goal is to introduce a general framework for these tasks and prove formally how both (recognition and learning) can be achieved. We show that both tasks can be accomplished even in presence of noise. For learning, we analyze Oja's rule formally, a well-known biologically-plausible rule for adjusting the weights of synapses. We complement the learning results with lower bounds asserting that, in order to recognize concepts of a certain hierarchical depth, neural networks must have a corresponding number of layers.

==> lowerbound_intuition.tex <==
\section{Lower Bounds}\label{sec:lowerbounds}

\snote{I think we probably could extend to a neuron model with strengths instead of just firing indicators.  Basically, by replacing the sums of weights by dot products.}

Here we give three lower bound theorems describing limitations on the number of layers needed to recognize concept hierarchies with particular numbers of levels.
%
First, \autoref{thm:imposs-2-vs-1}, says that a network $\mathcal N$ with maximum layer $1$ cannot recognize a concept hierarchy $\mathcal C$ with maximum level $2$.
This bound depends only on the requirement that $\mathcal N$ should recognize $\mathcal C$ according to our definition for noisy recognition in \sref{Definition}{def:noisyrecognition}. 
That definition says that the network must tolerate bounded noise, as expressed by the ratio parameters $r_1$ and $r_2$.  Our result assumes reasonable constraints on the values of $r_1$ and $r_2$.
 
\autoref{thm:imposs-3-vs-2}, extends \autoref{thm:imposs-2-vs-1} by showing that a network $\mathcal N$ with maximum layer $2$ cannot recognize a concept hierarchy $\mathcal C$ with maximum level $3$.
In addition to the basic definition of noisy recognition, this result requires a new "non-interference" assumption for concept representations in the network.  This assumption seems to be reasonable, in that it is guaranteed by our learning algorithms in \autoref{sec:algorithms_learning}; however, it would be preferable to weaken it to, say, a simple limitation on the number of neurons in the network, a task that we leave for future work.
%
\nnote{Verify this, add a lemma "for later use" at the end of Section 6 that we can cite here.  This would be a nice story, using a fact that is true about our (noise-free) learning algorithm in the proof of a lower bound for recognition.} 
%
\autoref{thm:imposs-general} generalizes the first two theorems to arbitrary numbers of levels and layers. 
The heart of the proof of \autoref{thm:imposs-general} is  \autoref{lem:imposs-general}, which considers a particular network $\mathcal N$ and concept hierarchy $\mathcal C$, where $\mathcal N$ recognizes $\mathcal C$.  
It says that, for any $\ell$, the representation of any level $\ell$ concept must be in a layer $\geq \ell$.  
The proof is by induction on $\ell$.
As for \autoref{thm:imposs-3-vs-2}, these results require the new  "non-interference" assumption.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Assumptions for the lower bounds}
\label{sec: lower-bound-assumptions}

\nnote{Various little rewrites in this subsection.}
Here we list the assumptions that we use for our lower bounds.
These assumptions are stated for a particular concept hierarchy $\mathcal C$, with concept set $C$, to be $(r_1,r_2)$-recognized by a particular network $\mathcal N$.
The first three properties are already required by the definition of the noisy recognition problem.
They are enough to prove \autoref{thm:imposs-2-vs-1}.

\begin{enumerate}
    \item  Every concept $c \in C$ has a unique designated neuron $rep(c)$ in the network.  (In general, it might be in any layer, regardless of the level of $c$.)
    \item  Let $B$ be any subset of $C_0$.  If $c \in supported_{r_2}(B)$, then presentation of $B$ results in firing of $rep(c)$ at time $t+layer(rep(c))$.
    \item  Let $B$ be any subset of $C_0$.  If $c \notin supported_{r_1}(B)$, then presentation of $B$ does not result in firing of $rep(c)$ at time $t+layer(rep(c))$.
\end{enumerate}

The fourth property is new, and used only for \autoref{thm:imposs-3-vs-2} and \autoref{thm:imposs-general}.
This property is an attempt to rule out extraneous firing caused by mixing inputs that belong to different higher-level concepts.
Stated informally:  showing several level $\ell$ concepts simultaneously does not trigger any additional firing at layers $0,\ldots,\ell$ of the network besides what we would get by presenting the sets one at a time.
\nnote{Technically, it says a bit more---the sets of triggered neurons are also disjoint.}

\begin{enumerate}[\hspace{0.45cm}4.]
    \item \emph{Non-interference:}    
Fix any $\ell \geq 1$.  
Consider any subset $B$ of the level $\ell$ concepts in $\mathcal C$.  
For each $b \in B$, let $N(b)$ be the set of neurons at layers $1,\ldots,\ell$ whose firing is triggered by showing $b$.\footnote{A note about timing:  When we say that the firing of a neuron $u$ is triggered by presenting a set of level $0$ concepts at time $t$, we mean that this firing occurs at time exactly $t+layer(u)$.}
Let $N$ be the set of neurons at layers $1,\ldots,\ell$ whose firing is triggered by showing all the concepts in $B$ at the same time.  
Then all the $N(b)$ sets are disjoint, and $N = \bigcup_{b \in B} N(b)$.
\end{enumerate}
\nnote{Here is where I found two problems. First, in order to make the sums work out right, I needed to add disjointness.  That seems fine.

Second, the assumption was too strong as stated since it talked about firing at "all layers".  But in our learning algorithms, showing multiple level $\ell$ concepts together can indeed cause new firing at level $\ell+1$, besides what we would get if these concepts where shown individually.  But what we need I think is just that we don't get anything different at level $\ell$ (or below).  So I added the qualifier $\leq \ell$.  I modifyied the last two proofs (slightly) to reflect this.  Needs checking.

Future work could be to try to weaken this assumption.
Caution:  If we don't have any such noninterference assumption then the lower bound doesn't hold.  Consider a 2-layer network in which we have EVERY allowable combination of inputs feeding into a dedicated layer 1 neuron.  That is a huge number of combinations of course, but it's still possible.  Then a layer 2 neuron can have incoming edges from all of these dedicated neurons, and a firing threshold of 1.  We might look for other assumptions that would preclude such trivial (expensive) solutions, in particular, bounding the number of neurons in the network.
}
%
\nnote{We assume throughout the paper that firing proceeds layer-by-layer, each layer at one time.  So when we talk about a neuron $u$ at level $\ell$ being triggered to fire, we mean that this occurs at time $t+layer(u)$, where $t$ is the time when the triggering set of level $0$ concepts is presented.
We might need to clarify this timing issue in other definitions and claims.  Here, I added a footnote.}
%
\nnote{Notational awkwardness in the statement of Property 4:  I am using the letter $B$ here for layer $\ell$ concepts, $\ell \geq 1$, whereas in the other three properties and elsewhere, we use $B$ for the level $0$ concepts that are presented.  We might end up changing the letter we use at some point, but now it's used it too many places in the lower bound proofs for me to want to do this right now.}
%

%
Note that all of the above assumptions hold for our learning algorithms. While they are natural, it is still possible that there might be other learning algorithms that do not satisfy these assumptions. \fnote{I've added the last sentence, but I'm not sure if we should keep it or not.}

Throughout this section, we assume the model presented in \autoref{sec:datamodel} and~\autoref{sec:networkmodel}.
Furthermore, since we are considering recognition only, and not learning, we assume that the $engaged$ state components are always equal to $0$.
%
\nnote{We are using a simplified version of our general model, simpler than what we allow for our algorithmic results.  Namely, neuron states are just binary `firing status" values, representing whether the neuron is firing or not at a particular time.  And we have no extra facilities such as WTA modules, just neurons arranged in layers.  This corresponds to the basic SNN model of Musco et al, ITCS paper 2017, new version in arXiv 2019, my composition paper 2018.}
%
Also throughout this section, we assume that $r_1$ and $r_2$ satisfy the following constraints:
\begin{enumerate}
    \item $0 \leq r_1 \leq r_2 \leq 1$.
    \item $r_1 k$ is not an integer; define $r_1'$ so that $r_1' k = \lfloor r_1 k \rfloor$.
    \item Define $r_2'$ so that $r_2' k = \lceil r_2 k \rceil$.
    \nnote{I think here it's OK to allow the case where $r_2' = r_2$.}
    \item $(r_2')^2 \leq 2 r_1' - (r_1')^2$.
\end{enumerate}
For example, for $k = 10$, $r_1 = .51$ and $r_2 = .8$ satisfy these conditions.  Or $r_1 = \frac{1}{3}$ and $r_2 = \frac{2}{3}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impossibility for recognition for two levels and one layer}
\label{sec:imposs-2-levels-1-layer}

\nnote{Various little rewrites.}
We consider an arbitrary concept hierarchy $\mathcal C$ with maximum level $2$ and concept set $C$.
%
We assume a  (static) network $\mathcal N$ with maximum layer $1$, and total connectivity from layer $0$ neurons to layer $1$ neurons.
%
For such a network and concept hierarchy, we get a contradiction to the noisy recognition problem  in \autoref{sec:prob-recog}, for any values of $r_1$ and $r_2$ that satisfy the constraints given in \autoref{sec: lower-bound-assumptions}.
%
For the problem requirements in this section, we use only Assumptions 1-3 from \autoref{sec: lower-bound-assumptions}.

\begin{theorem}
\label{thm:imposs-2-vs-1}
Assume that $\mathcal C$ has maximum level $2$ and $\mathcal N$ has maximum layer $1$.
Assume that $r_1, r_2, r_1', r_2'$ satisfy the constraints in \autoref{sec: lower-bound-assumptions}.
Then $\mathcal N$ does not recognize $\mathcal C$, according to Assumptions 1-3.
\end{theorem}
The proof can be found in \autoref{sec:lbproofs}
\fnote{The good thing is that for this case, $\ell=2$, no neurons fires with rates that differ from $0$ and $1$, since by definition the input neurons always have binary values. In principle the layer 1 neurons could have different weights, but that's not important here at all! Note that for $\ell>2$, all of this is no longer true.}

\nnote{I wondered about moving this lower bound proof to the main body.  But all the other technical material about the algorithms is in the Appendix, so that would not work well.  Also, we will have a space problem.  So I'm leaving this alone.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impossibility for recognition for three levels and two layers}
\label{sec: imposs-3-levels-2-layers}

\nnote{If we want to extend this result, and the general one, to allow neurons at layers $\geq 1$ to fire with different strengths, we will probably need an extension to Assumption 4 saying that the firing rates, as well as which neurons are firing, do not change when we present together.}

Now we consider another special case result, for three levels and two layers, before moving on in the next section to the general case of $\lmax$ levels and $\lmax-1$ layers.
Now we assume an arbitrary concept hierarchy $\mathcal C$ with maximum level $3$, and a network $\mathcal N$ with maximum layer $2$ and total connectivity between each consecutive pair of layers.
%
For such a network and concept hierarchy, we get a contradiction to the noisy recognition problem definition, for any values of $r_1$ and $r_2$ that satisfy the constraints given in \autoref{sec: lower-bound-assumptions}. 
For the problem requirements here, we use Assumptions 1-4 from \autoref{sec: lower-bound-assumptions}. 

\begin{theorem}
\label{thm:imposs-3-vs-2}
Assume that $\mathcal C$ has maximum level $3$ and $\mathcal N$ has maximum layer $2$.
Assume that $r_1, r_2, r_1', r_2'$ satisfy the constraints in \autoref{sec: lower-bound-assumptions}.
Then $\mathcal N$ does not recognize $\mathcal C$, according to Assumptions 1-4.
\end{theorem}
The proof can be found in \autoref{sec:lbproofs}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impossibility for recognition for $\lmax$ levels and $\lmax-1$ layers}

We now generalize the results of Sections~\ref{sec:imposs-2-levels-1-layer} 
and~\ref{sec: imposs-3-levels-2-layers} to arbitrary numbers of levels.
Now we assume an arbitrary concept hierarchy $\mathcal C$ with maximum level $\lmax$, and a network $\mathcal N$ with maximum layer $\ell'_{max}$ and total connectivity between consecutive layers.
Again we get a contradiction to the noisy recognition problem definition, for any values of $r_1$ and $r_2$ satisfying the constraints given in \autoref{sec: lower-bound-assumptions}. 
For the problem requirements here, we use Assumptions 1-4 from \autoref{sec: lower-bound-assumptions}.

\begin{theorem}
\label{thm:imposs-general}
Assume that $\ell'_{max} < \lmax$, that is, that the network $\mathcal N$ has fewer layers than the number of levels in the concept hierarchy $\mathcal C$.
Assume that $r_1, r_2, r_1', r_2'$ satisfy the constraints in \autoref{sec: lower-bound-assumptions}.
Then $\mathcal N$ does not recognize $\mathcal C$, according to Assumptions 1-4.
\end{theorem}

The proof of \autoref{thm:imposs-general} borrows ideas from that of \autoref{thm:imposs-3-vs-2}.  
However, instead of a case analysis as before, we would like to use induction on the level numbers. For this, we extract a lemma about where the $reps$ of different concepts may appear in a single network.  For this lemma (unlike in the theorem), we do not assume any particular relationship between $\lmax$ and $\ell'_{max}$.

\begin{lemma}
\label{lem:imposs-general}
Suppose that $\mathcal N$ recognizes $\mathcal C$, according to Assumptions 1-4.
Then for every $\ell, 1 \leq \ell \leq \lmax$, and for any level $\ell$ concept $c \in C$, $rep(c)$ is in a layer $\geq \ell$.
\end{lemma}
The proof can be found in \autoref{sec:lbproofs}.
Using \autoref{lem:imposs-general}, we can now prove the main theorem:

\begin{proof}[Proof of \autoref{thm:imposs-general}]
Assume that $\ell'_{max} < \lmax$, that is, that $\mathcal N$ has fewer layers than the number of levels in $\mathcal C$.
Assume for contradiction that $\mathcal N$ $(r_1,r_2)$-recognizes $\mathcal C$.

Fix any level $\lmax$ concept $c$.  Then by \autoref{lem:imposs-general}, $rep(c)$ must be in a layer $\geq \lmax$.  But this is impossible since $\mathcal N$ has strictly fewer than $\lmax$ layers.
\end{proof}

